Hindsight Bias in Clinical Temporal Reasoning: How Future Data Exposure Affects Large Language Model Judgment

Clinical decisions are prospective, but clinical language models are often evaluated on retrospective records that reveal the final diagnosis, treatment response, and outcome. Such evaluations may reward the use of future information rather than reasoning under the uncertainty present at the decision point. We introduce a paired benchmark for measuring outcome-conditioned shifts consistent with hindsight bias in clinical temporal reasoning. It contains 171 case reports from the PubMed Central Open Access Subset---40 sepsis and 131 GLP-1/diabetes cases---represented as both textual narratives and human-annotated and LLM-generated textual time series (TTS). For each case, questions are tied to a clinically meaningful cutoff and paired with a prospective reference answer and an outcome-consistent \emph{hindsight trap}. Models answer each question using either a TTS truncated at the cutoff or the complete timeline; additional conditions vary the narrative source (original or synthetic) and TTS annotation source (human or LLM). We evaluate accuracy (Acc), hindsight trap rate (HTR), answer instability rate (AIR), and hindsight bias rate (HBR), each of which captures different signals of hindsight bias. Across GPT 5.6 Sol, Gemma 4, GLM 5.2, and Opus 5, full timeline exposure produces consistent hindsight-sensitive shifts, while temporal masking reduces bias without lowering accuracy.

==> draft_scratch/discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion}
\label{sec:discussion}

\paragraph{Principal findings}
This study introduces a paired benchmark for testing whether access to later clinical information changes a model's judgment about a fixed case. The provisional results show a consistent qualitative pattern in the direct TTS-only comparison: complete-trajectory exposure increased attraction to an outcome-consistent hindsight trap across both clinical cohorts and both TTS annotation sources, whereas changes in aggregate accuracy were smaller and directionally mixed. \textcolor{blue}{TBD: Replace this sentence with the final headline effect sizes, confidence intervals, number of models showing the effect, and conditional HBR range.}

This metric pattern matters because accuracy alone does not identify the direction of a response change. A model may preserve high average accuracy while reversing a subset of prospectively correct answers after later information is revealed. Conversely, an answer may change because later evidence legitimately resolves uncertainty or corrects an earlier error. By reporting Acc, HTR, AIR, HBR, and the full transition decomposition together, the benchmark separates nondirectional instability and beneficial updating from movement specifically toward a predefined outcome-consistent alternative.

\paragraph{Relation to prior work}

Our findings extend prior demonstrations of hindsight sensitivity in paired clinical vignettes \cite{wang2024cognitivebias,degany2025o1bias} from small, hand-crafted scenarios to temporally structured trajectories derived from real case reports. The design is also related to ex-ante temporal-leakage evaluation \cite{liu2026exante}, but differs by defining a clinically meaningful cutoff, a prospective reference answer, and an item-specific hindsight trap for the same patient trajectory. \textcolor{blue}{TBD: Add the final comparison with any clinician baseline or counterfactual-outcome experiment, if completed.}

The results should not be interpreted as evidence that a language model experiences the same psychological mechanism as a human clinician. Rather, they identify an operationally similar failure mode: a judgment about an earlier state becomes more consistent with the known outcome after later information is exposed. This distinction is important for both scientific precision and clinical deployment.

\paragraph{Representation and annotation source}
The largest provisional masked--full differences occurred when the TTS was the only patient-specific input. In narrative-containing conditions, the complete retrospective narrative was identical across the pair, leaving the later course visible even when the accompanying TTS was truncated. The smaller paired effects in those conditions are therefore consistent with reduced separation between the information states, not necessarily with a protective effect of narrative prose. A clean comparison of structured and narrative representations requires generating each narrative from the corresponding masked or full TTS rather than reusing one full-trajectory narrative.

The directional HTR effect appeared in both human and LLM-generated TTS, suggesting that it is not unique to one annotation source. At the same time, differences in AIR and $\Delta$Acc indicate that the two TTS sources are not interchangeable. Event granularity, timing, retrospective labels, and cutoff alignment can change the evidence available to the model. \textcolor{blue}{TBD: Update this interpretation after the exact event-aligned subset and matched-information representation ablations are complete.}

\paragraph{Implications for clinical AI evaluation}

The benchmark highlights a general evaluation risk. Retrospective clinical records routinely contain information unavailable at the time of the decision being evaluated. If a model is asked to assess an earlier diagnosis, risk estimate, or treatment decision while seeing the complete episode, strong performance may partly reflect access to later evidence rather than reasoning under the original uncertainty. Evaluation datasets intended to approximate prospective use should therefore enforce the information boundary in the input itself.

A practical implication is that hard temporal masking may be more reliable than asking a model to ignore later information. \textcolor{blue}{TBD: Replace this conditional statement with the observed comparison among hard masking, explicit prospective instruction, and any boundary-marking prompt. If prompting substantially closes the gap, describe it as a partial mitigation rather than assuming that masking is always necessary.} The benchmark can also be used as an audit: systems can be compared not only on final-answer accuracy, but on how often later information induces correct-to-trap reversals.

\paragraph{Limitations}
Several limitations constrain the interpretation of the study. First, the construct requires a question whose target remains fixed at an earlier clinical reference point. \textcolor{blue}{TBD: In the current implementation, the reference time is hidden from the answering model and questions are intentionally unanchored. If the explicit-anchor rerun is adopted, replace this sentence with the final anchor design and report whether the effect persists. Otherwise, describe the primary outcome conservatively as outcome-conditioned answer distortion rather than definitive hindsight bias.}

Second, temporal masking is only valid when the cutoff excludes all information unavailable at the reference point. Event time may differ from recognition or information-availability time, and retrospectively written event descriptions can themselves encode later interpretations. \textcolor{blue}{TBD: State the final cutoff semantics, whether tied cutoff events are retained or excluded, how retrospective labels were handled, and the fraction of questions passing manual leakage review.}

Third, questions, prospective answers, and hindsight traps are generated by an LLM. This enables scalable paired evaluation but may introduce unsupported answers, implausible traps, option artifacts, or generator-specific phrasing. \textcolor{blue}{TBD: Report the clinical-review protocol, retained-item rate, inter-rater agreement, and results restricted to clinician-approved questions. If full clinical validation is not completed, state that generator-derived targets limit claims of clinical validity.}

Fourth, human and LLM TTS may differ in event granularity and timing. Applying a numeric cutoff derived from one representation to another can expose different clinical information. \textcolor{blue}{TBD: Report event-level alignment coverage and make the aligned subset the primary human-versus-LLM TTS comparison.}

Fifth, free-response evaluation depends on an LLM judge and may inherit judge inconsistency or same-family preference. Structured questions avoid this source of uncertainty, but they may simplify clinically nuanced judgments. \textcolor{blue}{TBD: Add clinician and second-judge agreement and summarize whether structured-only results support the same conclusion.}

Sixth, published case reports are retrospective, selectively reported, and enriched for unusual or educational presentations. They do not reproduce the prevalence, documentation practices, or operational constraints of routine EHR data. Some reports may also have appeared in model pretraining corpora, creating a risk of case memorization. \textcolor{blue}{TBD: Report publication-year and contamination sensitivity analyses, removal of identifying metadata, and results on paraphrased or counterfactual subsets if available.}

Seventh, the two cohorts differ in many respects beyond temporal duration, including disease process, care setting, narrative style, event density, and outcome type. The imbalance of 40 sepsis and 130 GLP-1/diabetes cases further limits direct cohort comparisons. Cohort differences should therefore be interpreted as heterogeneity across clinical settings, not as a causal effect of clinical tempo.

Finally, \textcolor{blue}{TBD: state the final number and diversity of answering models, whether all planned ablations were completed, and the extent to which mutable API versions limit reproducibility.} The paired design establishes sensitivity to added information, but without an outcome-only or counterfactual manipulation it cannot fully separate the causal effect of outcome knowledge from the effect of other clinically informative post-cutoff evidence.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}
\label{sec:conclusion}

We introduced a paired benchmark for evaluating whether later clinical information changes a model's answer about an earlier decision point. By combining time-masked and complete trajectories with prospective reference answers and outcome-consistent traps, the benchmark separates ordinary accuracy, nondirectional instability, beneficial updating, and harmful correct-to-trap reversals. \textcolor{blue}{TBD: Insert the final headline result, including the range of $\Delta$HTR and conditional HBR across models, cohorts, and TTS sources.} These findings motivate time-appropriate input construction and explicit outcome-sensitivity auditing when clinical language models are evaluated retrospectively.

==> draft_scratch/methods.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Methods}
\label{sec:methods}

\subsection{Study design and data source}
\label{sec:data}

We designed a paired, within-question evaluation to measure how access to later clinical information changes a model's answer about a fixed case. For each question, the model was evaluated under a \emph{masked} condition containing TTS events no later than a question-specific cutoff and a \emph{full} condition containing the complete TTS. Because the clinical question and all pre-cutoff information were held fixed within each pair, differences between the two responses quantify sensitivity to post-cutoff information.

Cases were drawn from the PubMed Central Open Access (PMC OA) Subset provided by \cite{nlm2025pmcoa}. We used two cohorts comprising 171 case reports: 40 sepsis cases and 131 GLP-1/diabetes cases. The sepsis cohort builds on a previously constructed collection of time-localized sepsis case reports \cite{noroozizadeh2026sepsistts}. We selected the two cohorts to evaluate the benchmark across contrasting clinical trajectories: comparatively dense, acute-care episodes in sepsis and more heterogeneous longitudinal trajectories in GLP-1/diabetes. We treat between-cohort comparisons as tests of robustness across clinical settings rather than as a causal test of disease tempo.

\textcolor{blue}{TBD: Describe the case-retrieval dates and queries, publication window, inclusion and exclusion criteria, duplicate handling, language restrictions, and the procedure used to select the final 40 sepsis and 130 GLP-1/diabetes reports.}

\subsection{Clinical representations}
\label{sec:representations}

Each case $i$ was represented by its original case-report narrative $N_i$ and by two textual time series (TTS): a human-annotated TTS $T_i^{\mathrm{H}}$ and an independently generated LLM TTS $T_i^{\mathrm{L}}$. A TTS is a sequence
\begin{equation}
T_i^{s}=\{(e_{ij}^{s},t_{ij}^{s})\}_{j=1}^{n_i^{s}}, \qquad s\in\{\mathrm{H},\mathrm{L}\},
\end{equation}
where $e_{ij}^{s}$ is a clinical event and $t_{ij}^{s}$ is its normalized relative time in hours. The files were stored as CSV tables with \texttt{event} and \texttt{time} columns. Rows were not assumed to appear in chronological order; the numeric \texttt{time} field was treated as the authoritative temporal signal. This representation preserves the distinction between narrative order and clinical event order, which may diverge in retrospectively written case reports.

We additionally constructed a synthetic narrative $S_i$ from a full TTS. The generation prompt instructed the model to convert the timeline into a coherent clinical narrative, preserve only information explicitly supported by the TTS, avoid unsupported causal or diagnostic inferences, and express timing relative to nearby events where possible. Synthetic narratives were used to test whether results depended on the original case-report prose or persisted under an independently reconstructed narrative representation.

\textcolor{blue}{TBD: Describe the human TTS annotation protocol, annotator qualifications, quality-control or adjudication process, time-normalization rules, and inter-annotator agreement if available. Also specify the model, prompt, decoding settings, and validation procedure used to generate the LLM TTS.}

\textcolor{blue}{TBD: Confirm the synthetic-narrative generator and version and whether distinct synthetic narratives will be generated from human and LLM TTS. In the current repository, one full-TTS-derived synthetic narrative is reused within the paired masked/full comparison.}

\subsection{Question construction}
\label{sec:question_generation}

Questions were generated with GPT-5.6 from the joint input of the original narrative $N_i$ and the human TTS $T_i^{\mathrm{H}}$. The generator produced exactly ten questions per case as a schema-constrained JSON array. Outputs failing schema validation were returned to the generator for up to one repair attempt. With 170 cases, this procedure yields 1,700 questions.

Each question $q$ contains a visible component---the question text, response format, and answer options when applicable---and hidden evaluation metadata: an implicit clinical reference time, an early cutoff event and numeric cutoff time $c_q$, a prospective reference answer $a_q^*$, an outcome-consistent hindsight-trap answer $a_q^{\mathrm{trap}}$, and a brief explanation of the post-cutoff information that makes the trap attractive. The trap was defined as a specific answer that is not supported by the intended pre-cutoff evidence but may appear more compelling after the subsequent diagnosis, treatment response, or outcome is known. For questions designed only to assess factual accuracy, the trap fields were null.

The generation prompt targeted three evaluation categories. \texttt{accuracy} questions were intended to have a verifiable answer and low hindsight sensitivity; \texttt{hindsight\_bias} questions targeted judgment-based assessments for which later information could alter perceived likelihood, severity, causality, or appropriateness; and \texttt{both} questions combined a prospectively defensible reference answer with a plausible hindsight trap. Each case was targeted to contain two \texttt{accuracy}, three \texttt{hindsight\_bias}, and five \texttt{both} questions, corresponding to 340, 510, and 850 questions, respectively.

Questions used free-response, four-option multiple-choice, and true/false formats. Multiple-choice questions were further labeled as categorical or ordinal. For ordinal items, options used explicit ranges rather than qualitative labels, and the prompt placed the reference answer and trap at maximally separated positions on the four-point scale. The generator was instructed to create no more than two questions of any one reasoning type per case, with candidate types including likelihood estimation, severity assessment, causal attribution, treatment appropriateness, diagnostic classification, and temporal ordering. It was also instructed to avoid questions about the TTS representation itself and to omit an explicit temporal reference from the visible question, so that prospective reasoning was induced by the available context rather than by an overt instruction.

The generator-supplied $a_q^*$ served as the benchmark reference answer, while $a_q^{\mathrm{trap}}$ served as the directional error target. Automated schema checks verified the required fields, response format, number and labeling of multiple-choice options, and target-specific presence of trap fields. Cutoff times were required to parse as finite numeric values during masking.

\textcolor{blue}{TBD: Add the final clinical review protocol and report the number of questions retained after review. At minimum, review should assess prospective answerability, correctness of $a_q^*$, plausibility and distinctness of $a_q^{\mathrm{trap}}$, cutoff validity, option validity, and post-cutoff leakage.}

\subsection{Temporal masking and cutoff position}
\label{sec:masking}

For every question, the generator supplied a numeric cutoff $c_q$ in the same time coordinate used by the human TTS. Given a TTS $T_i^s$, the masked representation was constructed as
\begin{equation}
T_{iq,\mathrm{masked}}^{s}
=
\{(e_{ij}^{s},t_{ij}^{s})\in T_i^{s}:t_{ij}^{s}\leq c_q\},
\label{eq:masking}
\end{equation}
while $T_{i,\mathrm{full}}^{s}=T_i^s$ retained the complete trajectory. Rows with designated missing time values were omitted during masking; non-missing event and cutoff times were required to parse as finite numeric values. The same numeric cutoff was applied to human and LLM TTS so that both sources were evaluated at the same nominal point in the case trajectory.

\textcolor{blue}{TBD: Report event-level alignment between the human and LLM TTS at each cutoff and define how unmatched cutoffs are handled. Applying the same numeric cutoff to both sources guarantees only a common nominal time, not identical visible clinical information.}

\textcolor{blue}{TBD: Confirm the boundary convention before the final rerun. The current implementation retains events satisfying $t\leq c_q$, whereas the generation prompt describes the cutoff event as the first event that should be hidden. The manuscript and code must consistently define $c_q$ as either the last visible event or the first hidden event.}

Because absolute case durations can be dominated by remote historical or follow-up events, we characterized each cutoff by its ordinal location in the human TTS. After sorting valid TTS rows by numeric time and preserving source order within ties, let $k_q\in\{1,\ldots,n_i\}$ be the chronological index matching the cutoff. We define
\begin{equation}
\operatorname{RelPos}(q)=\frac{k_q-1}{n_i-1},
\label{eq:relpos}
\end{equation}
where 0 denotes the first recorded event and 1 denotes the last. When multiple events shared a timestamp, event-text matching was used when possible; otherwise the first event at that time was selected. Questions whose cutoff could not be mapped to a TTS event were excluded from RelPos summaries but remained evaluable under the numeric masking rule.

\subsection{Experimental conditions}
\label{sec:conditions}

We evaluated seven input conditions (Table~\ref{tab:conditions}). Condition 0 provided the original narrative alone and was evaluated as an unpaired retrospective reference. Each remaining condition was run in matched full and masked variants. Conditions 1.x combined the original narrative with a human or LLM TTS; conditions 2.x provided the TTS alone; and conditions 3.x combined a synthetic narrative with a human or LLM TTS.

\begin{table}[t]
\centering
\small
\caption{Input conditions. H-TTS and L-TTS denote human and LLM textual time series, respectively. ``F/M'' indicates paired full and masked TTS variants.}
\label{tab:conditions}
\begin{tabular}{@{}cl@{}}
\toprule
\textbf{Condition} & \textbf{Model input} \\
\midrule
0   & Original narrative \\
1.1 & Original narrative + H-TTS (F/M) \\
1.2 & Original narrative + L-TTS (F/M) \\
2.1 & H-TTS only (F/M) \\
2.2 & L-TTS only (F/M) \\
3.1 & Synthetic narrative + H-TTS (F/M) \\
3.2 & Synthetic narrative + L-TTS (F/M) \\
\bottomrule
\end{tabular}
\end{table}

Within conditions containing a narrative (1.x and 3.x), the narrative component was held fixed and complete across the full and masked variants; only the TTS was changed. Consequently, conditions 2.1 and 2.2 provide the direct comparison between prefix-only and complete patient information, whereas conditions 1.x and 3.x test the incremental effect of changing the accompanying TTS when a retrospective narrative is already present. All conditions used the same generated question set.

\textcolor{blue}{TBD: Confirm that conditions 2.1 and 2.2 will be designated as the primary paired analysis and conditions 1.x and 3.x as representation/context ablations.}

\subsection{Answer generation}
\label{sec:answering}

The planned answering-model panel includes GPT-5.6, Gemma 4, and \textcolor{blue}{TBD: name and version of the third open-weight model}. For every model and condition, each question was answered independently. The model received only the visible fields \texttt{question}, \texttt{format}, and \texttt{options}; the reference time, cutoff, evaluation target, reference answer, trap, and trap explanation were withheld. Depending on the condition, the prompt supplied the original or synthetic narrative, the full or masked TTS, or both. Models were permitted to use general medical knowledge to interpret clinical language but were instructed not to invent patient-specific facts.

Responses were constrained to a JSON object with an \texttt{answer} and a concise \texttt{evidence} field. True/false responses were restricted to \texttt{true} or \texttt{false}; multiple-choice responses were required to reproduce one complete option; and free responses were limited to one to three sentences. The evidence field named the case event, finding, treatment, timestamp, or absence of information supporting the answer. No external tools, retrieval systems, or web access were provided.

\textcolor{blue}{TBD: Align the final answer prompts with the actual representation: the repository supplies CSV files whose stored row order may be non-chronological, whereas the current prompts describe a chronologically ordered JSON array. Rerun affected conditions if this prompt correction is adopted.}

\textcolor{blue}{TBD: Report the exact model identifiers and checkpoints, providers, API or serving frameworks, inference dates, context windows, temperatures, seeds when supported, maximum output tokens, quantization and hardware for open-weight models, and the number of failed or retried requests. The current saved answer artifacts do not independently encode all of this provenance.}

\subsection{Evaluation}
\label{sec:evaluation}

Let $a_{q,z}$ denote the model answer to question $q$ in visibility condition $z\in\{\mathrm{masked},\mathrm{full}\}$. We evaluate correctness against $a_q^*$ and directional movement toward $a_q^{\mathrm{trap}}$. Accuracy metrics are computed on \texttt{accuracy} and \texttt{both} questions, whereas trap-based metrics are computed on \texttt{hindsight\_bias} and \texttt{both} questions. Answer instability is defined for all paired questions. Condition 0 supports Acc and HTR but not paired metrics.

\paragraph{Structured responses.}
For true/false and categorical multiple-choice items, answers were canonicalized and scored by exact match. Define
\begin{equation}
C_q(a)=\mathbf{1}[a=a_q^*]
\end{equation}
and, when a trap is defined,
\begin{equation}
R_q(a)=\mathbf{1}[a=a_q^{\mathrm{trap}}].
\end{equation}
For ordinal multiple-choice questions, correctness remained exact, but trap attraction was graded according to movement from the correct option toward the trap. If $r(\cdot)$ denotes option rank, we used
\begin{equation}
R_q(a)=
\operatorname{clip}_{[0,1]}
\left(
\frac{[r(a)-r(a_q^*)]\,\operatorname{sgn}[r(a_q^{\mathrm{trap}})-r(a_q^*)]}
{\lvert r(a_q^{\mathrm{trap}})-r(a_q^*)\rvert}
\right).
\label{eq:ordinal_trap}
\end{equation}
With the correct answer and trap at opposite endpoints of a four-option scale, this produces scores in $\{0,\tfrac{1}{3},\tfrac{2}{3},1\}$.

\paragraph{Free-response judging.}
Free responses were evaluated by a GPT-5.6 LLM judge using structured JSON output. For each response, the judge received the question, $a_q^*$, $a_q^{\mathrm{trap}}$, the trap explanation, and the model's answer and evidence. It assigned correctness and trap-match scores in $\{0,0.5,1\}$, representing no, partial, or full semantic agreement. In the aggregate definitions below, these graded scores replace $C_q(a)$ and $R_q(a)$ for free-response items. A separate paired judging call received the masked and full responses and determined whether they were clinically equivalent and whether a correct masked answer shifted toward the trap under full context. The judge used a fixed task-level instruction but no item-specific rubric.

\textcolor{blue}{TBD: Specify the exact judge deployment and run date and add judge validation against a clinician-labeled subset and, if feasible, a second model judge. Report agreement and repeat the primary free-response analysis under alternate judge choices.}

\paragraph{Aggregate metrics.}
For an eligible question set $\mathcal{Q}$, we report the following means:
\begin{align}
\operatorname{Acc}_{z}
&=\frac{1}{\lvert\mathcal{Q}_{\mathrm{acc}}\rvert}
\sum_{q\in\mathcal{Q}_{\mathrm{acc}}} C_q(a_{q,z}),\\
\Delta\operatorname{Acc}
&=\operatorname{Acc}_{\mathrm{masked}}-\operatorname{Acc}_{\mathrm{full}},\\
\operatorname{HTR}_{z}
&=\frac{1}{\lvert\mathcal{Q}_{\mathrm{trap}}\rvert}
\sum_{q\in\mathcal{Q}_{\mathrm{trap}}} R_q(a_{q,z}),\\
\Delta\operatorname{HTR}
&=\operatorname{HTR}_{\mathrm{full}}-\operatorname{HTR}_{\mathrm{masked}}.
\end{align}
Thus, positive $\Delta\operatorname{Acc}$ indicates higher accuracy under masking, while positive $\Delta\operatorname{HTR}$ indicates greater attraction to the trap after the full trajectory is revealed.

The answer-instability rate (AIR) captures any paired answer change, regardless of direction:
\begin{equation}
\operatorname{AIR}
=\frac{1}{\lvert\mathcal{Q}_{\mathrm{pair}}\rvert}
\sum_{q\in\mathcal{Q}_{\mathrm{pair}}}
\mathbf{1}[a_{q,\mathrm{full}}\not\equiv a_{q,\mathrm{masked}}],
\end{equation}
where $\equiv$ denotes canonical equality for structured formats and clinical semantic equivalence according to the paired judge for free responses.

For all formats, define $I_q^{\mathrm{M-correct}}=1$ when the masked answer is fully correct (exact match for structured items or a judge correctness score of 1 for free responses), and 0 otherwise. For structured items, the per-question hindsight-bias score then credits movement of the full answer toward the trap:
\begin{equation}
\operatorname{HBR}_q
=I_q^{\mathrm{M-correct}}\,R_q(a_{q,\mathrm{full}}).
\label{eq:hbr}
\end{equation}
For free responses, $\operatorname{HBR}_q\in\{0,0.5,1\}$ is assigned directly by the paired judge under the same conceptual rule: credit is given only to the extent that the masked answer is correct and the full answer reflects the trap. We report the joint rate
\begin{equation}
\operatorname{HBR}_{\mathrm{joint}}
=\frac{1}{\lvert\mathcal{Q}_{\mathrm{both}}\rvert}
\sum_{q\in\mathcal{Q}_{\mathrm{both}}}\operatorname{HBR}_q
\end{equation}
and the conditional rate among questions answered correctly when masked,
\begin{equation}
\operatorname{HBR}_{\mathrm{cond}}
=
\frac{\sum_{q\in\mathcal{Q}_{\mathrm{both}}}\operatorname{HBR}_q}
{\sum_{q\in\mathcal{Q}_{\mathrm{both}}}I_q^{\mathrm{M-correct}}}.
\label{eq:hbr_cond}
\end{equation}
The denominator of $\operatorname{HBR}_{\mathrm{cond}}$ is reported with every estimate.

\textcolor{blue}{TBD: Confirm this final HBR eligibility rule and update the analysis script accordingly. The current repository summary includes accuracy-only and \texttt{hindsight\_bias} questions in the HBR denominator, whereas the equations above restrict HBR to \texttt{both} questions.}

We additionally decompose paired responses into correct-to-correct, correct-to-trap, correct-to-other-error, error-to-correct, trap-to-correct, and other/no-change transitions. This separates harmful hindsight-consistent reversals from beneficial use of additional information and nondirectional instability.

\subsection{Statistical analysis}
\label{sec:statistics}

All full-versus-masked comparisons are paired at the question level. Point estimates will be computed separately by model, cohort, TTS source, input condition, evaluation target, and response format. Because ten questions are generated from each case and are therefore not independent, uncertainty will be estimated with a case-clustered bootstrap: cases will be sampled with replacement, and all questions and paired responses belonging to each sampled case will be retained together. Confidence intervals will be calculated from the bootstrap distribution of Acc, HTR, AIR, HBR, and the paired differences $\Delta\operatorname{Acc}$ and $\Delta\operatorname{HTR}$.

The sepsis and GLP-1/diabetes cohorts will be analyzed separately. Any combined estimate will give equal weight to cohort-level estimates rather than pooling all questions, which would allow the larger GLP-1/diabetes cohort to dominate. Primary analyses will use question-level means with case-clustered uncertainty; case-macro averages, computed by first averaging within each case, will be reported as a sensitivity analysis.

\textcolor{blue}{TBD: Prespecify the number of bootstrap replicates, percentile versus bias-corrected confidence intervals, hypothesis tests, significance threshold, handling of multiple secondary comparisons, and whether the analysis will report $p$-values or confidence intervals only.}

\paragraph{Sensitivity and subgroup analyses.}
Planned analyses are restricted to (i) structured-response questions, which require no LLM judge; (ii) questions retained after clinical review; (iii) questions whose cutoff maps exactly to both TTS sources; (iv) the \texttt{both} category for which both prospective correctness and trap attraction are measurable; and (v) cases not used during prompt development. We will also stratify results by question format, evaluation target, TTS source, cohort, and RelPos tertile. \textcolor{blue}{TBD: retain and describe only robustness experiments completed before submission, including explicit temporal anchoring, same-input repeatability, question-only responses, chronological-order ablation, context-length placebo, and outcome-only or counterfactual suffix controls.}

% \subsection{Ethics and reproducibility}
% \label{sec:ethics}

% The study uses publicly available case reports from the PMC OA Subset and does not involve prospective patient recruitment or model deployment in clinical care. Article-level reuse remains subject to the license attached to each source report. We will release the question metadata, prompts, evaluation code, and derived outputs to the extent permitted by the underlying licenses, together with model and run provenance needed to reproduce the reported analyses.

% \textcolor{blue}{TBD: Insert the institution-specific IRB approval, exemption, or non-human-subjects determination and the final data/code availability statement required by ML4H.}

==> draft_scratch/results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results}
\label{sec:results}



\subsection{Benchmark composition}
\label{sec:results_composition}

The intended benchmark comprises 170 case reports and 1,700 questions: 400 questions from 40 sepsis cases and 1,300 questions from 130 GLP-1/diabetes cases. Under the prespecified 20/30/50 target allocation, the candidate set contains 340 \texttt{accuracy}, 510 \texttt{hindsight\_bias}, and 850 \texttt{both} questions. Table~\ref{tab:benchmark_composition} summarizes the working candidate set. \textcolor{blue}{TBD: Replace these candidate counts with the final post-quality-control counts, including the numbers retained after clinical review, cutoff validation, human--LLM TTS alignment, and removal of malformed or duplicated questions.}

\begin{table}[t]
\centering
\caption{\textbf{Working benchmark composition before final quality control.} Counts for the GLP-1/diabetes cohort use the provisional 130-case manifest described below.}
\label{tab:benchmark_composition}
\small
{\color{blue}
\begin{tabular}{@{}lrrr@{}}
\toprule
\textbf{Characteristic} & \textbf{Sepsis} & \textbf{GLP-1/diabetes} & \textbf{Total} \\
\midrule
Cases & 40 & 130 & 170 \\
Questions & 400 & 1,300 & 1,700 \\
\texttt{accuracy} & 80 & 260 & 340 \\
\texttt{hindsight\_bias} & 120 & 390 & 510 \\
\texttt{both} & 200 & 650 & 850 \\
Free response & 89 & 301 & 390 \\
Multiple choice & 190 & 603 & 793 \\
True/false & 121 & 396 & 517 \\
\bottomrule
\end{tabular}}
\end{table}

\textcolor{blue}{TBD: Confirm the final 130-case GLP-1/diabetes manifest. The current repository contains 131 evaluated GLP cases; for the provisional 130-case point estimates below, we exclude the single case whose question allocation differs from the intended 2/3/5 \texttt{accuracy}/\texttt{hindsight\_bias}/\texttt{both} distribution. Regenerate all results after the final case manifest is frozen.}

\subsection{Complete trajectories increased attraction to hindsight traps}
\label{sec:results_primary}

We first evaluated the direct temporal-masking comparison using TTS-only inputs (conditions 2.1 and 2.2). Table~\ref{tab:primary_results} presents provisional point estimates from the currently completed GPT-5.6 run. Across both cohorts and both TTS annotation sources, the hindsight-trap score was higher when the complete trajectory was available than when the TTS was masked at the question-specific cutoff.

\begin{table*}[t]
\centering
\caption{\textbf{Provisional GPT-5.6 results for the TTS-only paired conditions.} Values are percentages. $\Delta$Acc is masked minus full; $\Delta$HTR is full minus masked. HBR is recomputed on \texttt{both} questions to match Section~\ref{sec:evaluation}. H-TTS and L-TTS denote human-annotated and LLM-generated TTS. All values must be replaced after the final 40+130 case manifest, post-QC rerun, and case-clustered bootstrap.}
\label{tab:primary_results}
\scriptsize
{\color{blue}
\begin{tabular}{@{}llrrrrrrrrr@{}}
\toprule
\textbf{Cohort} & \textbf{TTS} & \textbf{Acc-M} & \textbf{Acc-F} & \textbf{$\Delta$Acc} & \textbf{HTR-M} & \textbf{HTR-F} & \textbf{$\Delta$HTR} & \textbf{AIR} & \textbf{HBR$_{\mathrm{joint}}$} & \textbf{HBR$_{\mathrm{cond}}$} \\
\midrule
Sepsis & H-TTS & 96.1 & 94.5 & +1.6 & 9.2 & 18.1 & +8.9 & 9.8 & 4.3 & 4.5 \\
Sepsis & L-TTS & 90.4 & 92.1 & $-$1.8 & 10.1 & 19.7 & +9.6 & 16.0 & 5.5 & 6.1 \\
GLP-1/diabetes & H-TTS & 95.5 & 94.6 & +0.9 & 9.2 & 16.8 & +7.7 & 10.6 & 4.0 & 4.2 \\
GLP-1/diabetes & L-TTS & 91.4 & 92.2 & $-$0.8 & 10.5 & 17.7 & +7.2 & 11.1 & 3.3 & 3.5 \\
\bottomrule
\end{tabular}}
\end{table*}

\textcolor{blue}{Provisional current-run result: revealing the complete human TTS increased HTR by 8.9 percentage points in sepsis and 7.7 points in the working 130-case GLP-1/diabetes set. Using LLM-generated TTS, the corresponding increases were 9.6 and 7.2 points. In contrast, $\Delta$Acc ranged from $-1.8$ to $+1.6$ points across these four comparisons, indicating that the directional shift toward the trap was not consistently reflected in aggregate accuracy. AIR ranged from 9.8\% to 16.0\%. Among \texttt{both} questions answered correctly under masking, provisional conditional HBR ranged from 3.5\% to 6.1\%.}

\textcolor{blue}{TBD: Add 95\% case-clustered bootstrap confidence intervals and prespecified significance tests for every estimate; replace the working GLP values after the 130-case manifest is confirmed; add the remaining answering models; and report the masked-correct denominator for every conditional HBR value.}

\begin{figure*}[t]
\centering
\fbox{\parbox[c][1.2in][c]{0.94\textwidth}{\centering
\textcolor{blue}{TBD: Insert the primary forest plot. Panel A should show $\Delta$HTR with 95\% case-clustered bootstrap intervals by model, cohort, and TTS source. Panel B should show conditional HBR or the correct-to-trap transition probability with its denominator. Include a vertical zero line and distinguish H-TTS from L-TTS.}}}
\caption{Paired effect of complete versus masked TTS exposure on trap attraction and harmful answer reversals.}
\label{fig:primary_effect}
\end{figure*}

\subsection{Narrative-containing conditions showed smaller paired differences}
\label{sec:results_representation}

Conditions 1.x and 3.x held a complete narrative fixed in both members of each pair and changed only the accompanying TTS. As expected from this design, their provisional masked--full differences were smaller than in the TTS-only conditions. \textcolor{blue}{In the current GPT-5.6 run, $\Delta$HTR across the four narrative-containing conditions ranged from 0.4 to 1.7 percentage points in sepsis and from 0.3 to 0.9 points in the working 130-case GLP-1/diabetes set, compared with 7.2--9.6 points in the TTS-only comparisons. AIR was approximately 3.3--4.3\% in the narrative-containing conditions, versus 9.8--16.0\% with TTS alone.}

These conditions should therefore be interpreted as representation or context-augmentation ablations rather than as clean prospective-versus-retrospective comparisons: later information remains available through the unchanged narrative even when the TTS is masked. \textcolor{blue}{TBD: Replace the ranges above with final estimates and confidence intervals and report all condition-level results in the appendix. If matched masked and full synthetic narratives are regenerated, add that clean representation comparison separately.}

\subsection{Consistency across cohorts, TTS sources, and models}
\label{sec:results_generalization}

The direction of the provisional TTS-only HTR effect was consistent across the acute sepsis cohort and the more longitudinal GLP-1/diabetes cohort, and across human and LLM-generated TTS. However, the accompanying changes in accuracy and AIR differed by TTS source, particularly in sepsis, indicating that annotation source may alter both the information retained before the cutoff and the general stability of the model response. We therefore interpret cohort and annotation-source comparisons as robustness analyses rather than as evidence that any difference is caused by disease tempo or annotation quality alone.

\textcolor{blue}{TBD: Report the full model panel and model-by-visibility, cohort-by-visibility, and TTS-source-by-visibility interaction estimates. State whether the direction of $\Delta$HTR replicates for every model, and identify any model or subgroup for which the confidence interval includes zero or reverses direction.}

\subsection{Question-level heterogeneity and answer transitions}
\label{sec:results_heterogeneity}

The aggregate metrics combine heterogeneous response formats and reasoning targets. The final analysis will therefore report structured-response questions separately from free responses, for which no LLM judge is required, and will stratify results by evaluation target, response format, reasoning category, and relative cutoff position. The transition decomposition will distinguish correct-to-trap reversals from correct-to-other-error changes, beneficial error-to-correct updates, trap-to-correct changes, and stable responses.

\textcolor{blue}{TBD: Insert the transition figure and report (i) the proportion of all paired questions that remain unchanged, (ii) correct-to-trap transitions, (iii) correct-to-other-error transitions, and (iv) error-to-correct transitions for each primary condition. Report results separately for structured and free-response questions and provide the complete transition matrices in the appendix.}

\textcolor{blue}{TBD: Report subgroup results by question format, evaluation target, reasoning type, and RelPos tertile. Explicitly test whether \texttt{accuracy} questions behave as a negative control, with minimal $\Delta$HTR and correct-to-trap movement.}

\subsection{Sensitivity analyses and construct-validity controls}
\label{sec:results_sensitivity}

The principal interpretation depends on showing that masked--full differences exceed ordinary response variability and are not explained solely by question wording, context length, event ordering, cutoff mismatch, or LLM judging. \textcolor{blue}{TBD: Report, in this order, (1) same-input repeatability, (2) structured-only results, (3) clinically reviewed questions, (4) exact human--LLM cutoff-aligned questions, (5) exclusion of prompt-development cases, (6) explicit prospective anchoring versus unanchored questions, (7) chronological versus source-order TTS, (8) question-only and context-length placebo baselines, (9) outcome-only versus non-outcome suffixes, and (10) counterfactual-outcome probes if completed. For each control, state whether the primary $\Delta$HTR and HBR conclusions remain materially unchanged.}

\textcolor{blue}{TBD: Add judge-validation results, including agreement between GPT-5.6, a second judge model, and clinician labels; repeat the free-response analysis under each judge; and report an analysis restricted to structured questions as the judge-free primary sensitivity result.}

\subsection{Qualitative examples}
\label{sec:results_examples}

\textcolor{blue}{TBD: Include two compact examples. The first should show a clinically defensible masked answer that changes toward the predefined trap after a decisive post-cutoff event is revealed. The second should show a beneficial update or a stable answer, demonstrating that the framework does not label every response change as hindsight bias. For each example, display the reference point, abbreviated masked context, relevant later event, question, reference answer, trap, masked answer, and full answer.}

==> images/teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}

